Soft-to-Hard Vector Quantization for End-to-End Learning Compressible Representations

We present a new approach to learn compressible representations in deep architectures with an end-to-end training strategy. Our method is based on a soft (continuous) relaxation of quantization and entropy, which we anneal to their discrete counterparts throughout training. We showcase this method for two challenging applications: Image compression and neural network compression. While these tasks have typically been approached with different methods, our soft-to-hard quantization approach gives results competitive with the state-of-the-art for both.

==> network_plot.tex <==
\definecolor{mycolor1}{rgb}{0.15700,0.24700,0.57300}%
\definecolor{mycolor2}{rgb}{0.11400,0.65500,0.18000}%
\definecolor{mycolor3}{rgb}{0.58400,0.10200,0.52500}%
\definecolor{mycolor4}{rgb}{0.82400,0.14500,0.19600}%
\definecolor{mycolor5}{rgb}{0.84300,0.38400,0.14900}%
\definecolor{mycolor6}{rgb}{0.00000,0.31400,0.31400}%
\definecolor{myBlack}{rgb}{0.00000,0,0}%
%
\begin{tikzpicture}
\begin{axis}[%
width=4.085in,
height=3.106in,
at={(0.769in,0.473in)},
scale only axis,
xmin=0,
xmax=7,
xtick={1,2,3,4,5,6},
xticklabels={{   1},{   5},{   10},{  25},{  50},{  101}},
xlabel={number of regressors / output neurons},
%ymin=27.5,
ymin=3,
ymax=4,
ylabel={MAE (years)},
    %axis background/.style={fill=white},
    %axis x line*=bottom,
%axis y line*=left,
legend style={at={(0.8,0.8)}, anchor=north,legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor2,ultra thick, solid,mark=triangle,mark options={solid},mark size=1.9pt]
  table[row sep=crcr]{%
2	3.955\\
3	3.505\\
4	3.353\\
5	3.318\\
6	3.444\\
};
\addlegendentry{DEX};

\addplot [color=mycolor3,ultra thick, solid,mark=triangle,mark options={solid},mark size=2.9pt]
  table[row sep=crcr]{%
2	3.2585\\
3	3.2373\\
4	3.2499\\
5	3.2816\\
6	3.2657\\
};
\addlegendentry{ARN (ours)};
\addplot [color=mycolor1,ultra thick, solid,mark=star,mark options={solid},mark size=2.9pt]
  table[row sep=crcr]{%
1	3.650\\
};
\addlegendentry{Regression};

\end{axis}
\end{tikzpicture}%
